Fixed-parameter tractability of Graph Isomorphism in graphs with an excluded minor

We prove that Graph Isomorphism and Canonization in graphs excluding a fixed graph $H$ as a minor can be solved by an algorithm working in time $f(H)\cdot n^{O(1)}$, where $f$ is some function. In other words, we show that these problems are fixed-parameter tractable when parameterized by the size of the excluded minor, with the caveat that the bound on the running time is not necessarily computable. The underlying approach is based on decomposing the graph in a canonical way into unbreakable (intuitively, well-connected) parts, which essentially provides a reduction to the case where the given $H$-minor-free graph is unbreakable itself. This is complemented by an analysis of unbreakable $H$-minor-free graphs, performed in a second subordinate manuscript, which reveals that every such graph can be canonically decomposed into a part that admits few automorphisms and a part that has bounded treewidth.

==> preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

\usepackage{amssymb,amsmath,mathrsfs}
\usepackage{soul}

\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}

\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}

\usepackage{graphics}
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}

\newcommand{\OO}{\mathcal{O}}
\newcommand{\cO}{\mathcal{O}}

\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{redrule}{Reduction Rule}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{reduction}{Reduction Rule}[section]
\newtheorem{conjecture}{Conjecture}[section]

\date{}
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  %
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}

\newcommand{\yes}{\textsf{Yes}}
\newcommand{\no}{\textsf{No}}
\newcommand{\yesinstance}{\yes-instance}
\newcommand{\noinstance}{\no-instance}
\newcommand{\tw}{\mathtt{tw}}
\newcommand{\NP}{\textsf{NP}}
\newcommand{\coNP}{\textsf{co-NP}}
\newcommand{\FPT}{\textsf{FPT}}
\newcommand{\XP}{\text{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}
\newcommand{\nil}{\ensuremath{\mathtt{nil}}}
\newcommand{\dist}{\ensuremath{\mathsf{dist}}}
\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}

\newcommand{\pdp}{\textsf{Planar Disjoint Paths}}

\newcommand{\bnd}{\partial}


==> smallCentersBackup.tex <==




\begin{lemma}\label{lem:smallCentersAlgorithm}
There exists an algorithm that takes as input a compactly colored graph $G$, a vertex set $D \subseteq V(G)$, an isomorphism invariant (with respect to $G$ and $D$) star decomposition $(T, \chi)$ of $G$ with central bag $b$ such that $D \subseteq \chi(b)$, and a compact locally weakly isomorphism invariant leaf-labeling $\{ \lambda_{\pi, \ell} \}$ of $(T, \chi)$. The algorithm runs in time $(|\chi(b)|)! \cdot n^{\cO(1)}$ and outputs for every permutation $\iota \colon D \rightarrow [|D|]$ a canonical labeling of $(G, \iota)$.
\end{lemma}

\begin{proof}
The algorithm iterates through all choices of a permutation $\gamma \colon \chi(b) \rightarrow [|\chi(b)|]$. For each choice of $\gamma$ the algorithm produces a labeling $\lambda$ of $G$ that coincides with $\gamma$ on $\chi(b)$. For each $\iota : D \rightarrow [|D|]$ the algorithm then outputs a  $\lambda$ that yields a lexicographically smallest labeled graph $(G, \lambda)$ over all the choices of $\gamma$ that coincide with $\iota$ on $D$. 
We note that because $(T, \chi)$ is isomorphism invariant with respect to $G$ and $D$, it is also isomorphism invariant with respect to $G$, $D$ and $\iota$.


Since picking a lexicographically first labeling is a weakly isomorphism invariant function, to prove correctness it suffices to show the construction of $\lambda$ is weakly isomorphism invariant with respect to $G$, $(T, \chi)$ the leaf labeling $\{ \lambda_{\pi, \ell} \}$ as well as with respect to $\gamma$. We now describe how the algorithm constructs $\lambda$ given $\gamma$.

The algorithm proceeds as follows. For each leaf $\ell$ define the permutation $\pi^\ell\colon \sigma(\ell)\to [|\sigma(\ell)|]$ (not to be confused with $\pi\langle\ell\rangle$) to be the unique permutation of $\sigma(\ell)$ so that $\pi(u) < \pi(v)$ if and only if $\gamma(u) < \gamma(v)$. We define $\lambda^\ell$ to be $\lambda_{\pi^\ell, \ell}$.
The algorithm sorts the leaves $\ell$ of $T$ according to the lexicographic ordering of the set of labels $\gamma( \sigma(\ell) )$. For leaves $\ell$ and $\ell'$ that are tied according to this order (so $\sigma(\ell) = \sigma(\ell')$) it breaks ties by picking first the lexicographically smallest of $G[\chi(\ell)]$ with labeling $\lambda^\ell$, and $G[\chi(\ell')]$ with labeling $\lambda^{\ell'}$. Note that if $\ell$ and $\ell'$ are still tied then $(\lambda^{\ell'})^{-1}\lambda^\ell$ is an isomorhism from  $G[\chi(\ell)]$ to $G[\chi(\ell')]$ that maps each vertex $v$ of $\sigma(\ell)$ to itself. 

The labeling $\lambda$ is defined as follows. For every vertex $v \in \chi(b)$ where $b$ is the central bag of $T$ we set $\lambda(v) = \gamma(v)$. For every leaf $\ell$ and every vertex $v$ in $\chi(\ell) \setminus \chi(b)$ we set $\lambda(v) = \lambda^ \ell(v) + ((n+1) \cdot p)$ where $p$ is the position of $\ell$ in the sorted order of leaves defined above.  The algorithm outputs $\lambda$ as the weakly isomorphism invariant (with respect to $G$ and $\gamma$) labeling of $G$. The algorithm clearly runs in time $(|\chi(b)|)! \cdot n^{\cO(1)}$ and outputs a  labeling of $G$. Thus to complete the proof it suffices to show that $\lambda$ is in fact weakly isomorphism invariant in $G$, $(T, \chi)$,  $\{ \lambda_{\pi, \ell} \}$ and $\gamma$.

Consider now a graph $\hat{G}$, with star decomposition $(\hat{T}, \hat{\chi})$ with central bag $\hat{b}$, leaf labeling $\{ \hat{\lambda}_{\hat{\pi}, \hat{\ell}} \}$ of  $(\hat{T}, \hat{\chi})$ and permutation $\hat{\gamma} : \hat{\chi}(\hat{b}) \rightarrow [|\hat{\chi}(\hat{b})|]$.
Suppose that there exists an isomorphism $\phi$ from $G$ to $\hat{G}$ that respects $(T, \chi)$,  $\{ \lambda_{\pi, \ell} \}$ and $\gamma$.
Specifically we assume that there exists an isomorphism $\phi_T$ from $T$ to $\hat{T}$ such that the following holds:
\begin{itemize}\setlength\itemsep{-.7pt}
\item For every $u \in V(G)$ and every $q \in V(T)$ we have $u \in \chi(q)$ if and only if $\phi(u) \in \phi_T(q)$. 
\item For every $u \in \chi(b)$ we have that $\gamma(u) = \hat{\gamma}\phi(u)$
\item For every leaf $\ell$ of $T$ and every permutation $\pi \colon \sigma(\ell) \rightarrow [|\sigma(\ell)|]$, let $\hat{\ell} = \phi_T(\ell)$ and let $\hat{\pi} \colon \hat{\sigma}(\hat{\ell}) \rightarrow [|\hat{\sigma}(\hat{\ell})|]$
be defined as $\hat{\pi}(u) = \pi\phi^{-1}(u)$ for every $u \in \hat{\chi}(\hat{\sigma}(\hat{\ell}))$.
Then $\hat{\lambda}_{\hat{\pi}, \hat{\ell}}^{-1}\lambda_{\pi, \ell}$ is an isomorphism from $G[\chi(\ell)]$  to $\hat{G}[\hat{\chi}(\hat{\ell})]$.
\end{itemize}



Let $\hat{\lambda}$ be the labeling produced by the algorithm on input $\hat{G}$, $(\hat{T}, \hat{\chi})$, $\{ \hat{\lambda}_{\pi, \hat{\ell}} \}$ when considering the permutation $\hat{\gamma}$. To prove that $\lambda$ is weakly isomorphism invariant it suffices to show that $\hat{\lambda}^{-1}\lambda$ is an isomorphism from $G$ to $\hat{G}$.
We have that  $\hat{\lambda}^{-1}\lambda$ coincides with $\hat{\gamma}^{-1}\gamma$, which in turn coincides with $\phi$, and therefore $\hat{\lambda}^{-1}\lambda$ is an isomorphism from $G[\chi(b)]$ to $\hat{G}[\hat{\chi}(\hat{b})]$. 




Let $\ell$ be an arbitrarily chosen leaf of $T$ and $p$ be the position of $\ell$ in the sorted list of leaves produced by the algorithm. Let $\hat{\ell}$ be the leaf in position $p$ in the sorted list of the leaves of $\hat{T}$. To prove that  $\hat{\lambda}^{-1}\lambda$ is an isomorphism from $G$ to $\hat{G}$ it is sufficient to prove that $\hat{\lambda}^{-1}\lambda$ is an isomorphism from $G[\chi(\ell)]$ to $\hat{G}[\hat{\chi}(\hat{\ell})]$. 


Since $\phi$ respects $\gamma$ we have that for every leaf $\ell'$ in $T$,  $\gamma \sigma (\ell') = \hat{\gamma}\hat{\sigma}\phi_T(\ell')$. 
Further, since $\phi$ is an isomorphism and the labelings $\{ \hat{\lambda}_{\hat{\pi}, \hat{\ell}} \}$ are locally weakly isomorphism invariant it follows that for every leaf $\ell'$ in $T$ the graph $G[\chi(\ell')]$ with labeling $\lambda^{\ell'}$ and the graph $\hat{G}[\hat{\chi}(\phi_T(\ell'))]$ with labeling $\hat{\lambda}^{\phi_T(\ell')}$ are equal.

Let now $\ell' = \phi_T^{-1}(\hat{\ell})$. Suppose $\sigma(\ell')$ is lexicographically larger than $\sigma(\ell)$, or $\sigma(\ell') = \sigma(\ell)$ and the graph $G[\chi(\ell')]$ with labeling $\lambda^{\ell'}$ is lexicographically larger than $G[\chi(\ell)]$ with labeling $\lambda^{\ell}$. Then, for every leaf $\ell''$ at position $p$ or smaller in the ordering of the leaves of $T$ we have that $\phi_T(\ell'')$ comes before $\phi_T(\ell') = \hat{\ell}$ in the ordering of the leaves of $\hat{T}$. But this contradicts that $\hat{\ell}$ is at position $p$ in this ordering. Similarly if $\sigma(\ell')$ is lexicographically smaller than $\sigma(\ell)$, or $\sigma(\ell') = \sigma(\ell)$ and the graph $G[\chi(\ell')]$ with labeling $\lambda^{\ell'}$ is lexicographically smaller than $G[\chi(\ell)]$ with labeling $\lambda^{\ell}$ then for every leaf $\ell''$ at position $p$ or larger in the ordering of the leaves of $T$ we have that $\phi_T(\ell'')$ comes before $\phi_T(\ell') = \hat{\ell}$ in the ordering of the leaves of $\hat{T}$. Again this  contradicts that $\hat{\ell}$ is at position $p$ in this ordering. We conclude that $\sigma(\ell') = \sigma(\ell)$ and that $G[\chi(\ell')]$ with labeling $\lambda^{\ell'}$ is equal to $G[\chi(\ell)]$ with labeling $\lambda^{\ell}$. 

Hence (by choice of $\ell' = \phi_T^{-1}(\hat{\ell})$) we have that $\hat{G}[\hat{\chi}(\hat{\ell})]$ with labeling $\hat{\lambda}^{\hat{\ell}}$ is equal to $G[\chi(\ell')]$ with labeling $\lambda^{\ell'}$ and therefore also to $G[\chi(\ell)]$ with labeling $\lambda^{\ell}$. 
Thus $(\hat{\lambda}^{\hat{\ell}})^{-1}\lambda^{\ell}$ is an isomorphism from $G[\chi(\ell)]$ to $\hat{G}[\hat{\chi}(\hat{\ell})]$. 
However, for vertices in $\sigma(\ell)$ we have $(\hat{\lambda}^{\hat{\ell}})^{-1}\lambda^{\ell}(v) = \hat{\gamma}^{-1}\gamma(v) = \hat{\lambda}^{-1}\lambda(v)$. On the other hand both $\ell$ and $\hat{\ell}$ are at position $p$ in their respective orderings. Therefore, for vertices in $\chi(\ell) \setminus \sigma(\ell)$ we have that $\lambda(v) = \lambda^{\ell}(v) + ((n+1) \cdot p)$, while for vertices in  $\hat{\chi}(\hat{\ell}) \setminus \hat{\sigma}(\hat{\ell})$ we have that $\hat{\lambda}(v) = \hat{\lambda}^{\hat{\ell}}(v) + ((n+1) \cdot p)$. Thus for vertices in $\chi(\ell) \setminus \sigma(\ell)$  it holds that $(\hat{\lambda}^{\hat{\ell}})^{-1}\lambda^{\ell}(v) =  \hat{\lambda}^{-1}\lambda(v)$. And so we can conclude that $\hat{\lambda}^{-1}\lambda(v)$  is an isomorphism from $G[\chi(\ell)]$ to $\hat{G}[\hat{\chi}(\hat{\ell})]$, completing the proof. 
\end{proof}
